Constraint LTL Satisfiability Checking without Automata

This paper introduces a novel technique to decide the satisfiability of formulae written in the language of Linear Temporal Logic with Both future and past operators and atomic formulae belonging to constraint system D (CLTLB(D) for short). The technique is based on the concept of bounded satisfiability, and hinges on an encoding of CLTLB(D) formulae into QF-EUD, the theory of quantifier-free equality and uninterpreted functions combined with D. Similarly to standard LTL, where bounded model-checking and SAT-solvers can be used as an alternative to automata-theoretic approaches to model-checking, our approach allows users to solve the satisfiability problem for CLTLB(D) formulae through SMT-solving techniques, rather than by checking the emptiness of the language of a suitable automaton A_{\phi}. The technique is effective, and it has been implemented in our Zot formal verification tool.

==> proof-corollary-shift-symbolic-models.tex <==
\begin{proof}
It is easy to see that relation $\symodels$ is not affected by
rewriting $\shiftleft$.
In fact, for atomic formulae $R(\alpha_1,\dots,\alpha_n)$ we have that
$\rho,i\symodels R(\alpha_1,\dots,\alpha_n)$ if, and only if,
$\shiftleft(\rho),i \symodels \shiftleft(R(\alpha_1,\dots,\alpha_n))$.
Let us suppose that for all assignments $v'$, we have $v'
\models_\D f(\rho(i))$ if, and only if, $v' \models_\D f(R)$.
Then, since $p$ is a rewriting of terms, the previous property is
preserved provided that assignment $f$ is replaced by a function
$f':\shiftleft(\terms(\phi)) \rightarrow A$, where $A$ is a set of fresh
variables (see Section \ref{section-symbolic}).
Standard temporal modalities are handled as for $\models$.
\end{proof}

==> proof-equisat-noY.tex <==
\begin{proof}
Let $s=\lfloor\phi \rfloor$. % and $\sigma$ be a model for $\phi$; i.e., $\sigma,0 \models \phi$.
We show that for all $i\geq 0$, $\sigma, i \models \phi \iFF \sigma, i+s \models p(\phi)$ by induction on the structure of the formula $\phi$.
%Let $i\geq 0$ be an instant of the model $\sigma$ and $\varphi$ a subformula of $\phi$.

\noindent
The {\bf base case} of the induction is given on the atomic formulae $\phi = R(\alpha_1
\dots \alpha_n)$.
Since $\sigma, i \models_\D
  \phi \iFF R(\sigma(i+|\alpha_1|, x_{\alpha_1}) ,\dots,
  \sigma(i+|\alpha_n|, x_{\alpha_n}))$, by shifting the instant $i$ of
  $s$ the satisfaction relation is $\sigma, i \models_\D
  \phi \iFF R(\sigma(i+s+|\alpha_1|-s, x_{\alpha_1}) ,\dots,
  \sigma(i+s+|\alpha_n|-s, x_{\alpha_n}))$.
Then, we can equivalently write
$\sigma, i \models_\D
  \phi \iFF R(\sigma(i+s+|p(\alpha_1)|, x_{\alpha_1}) ,\dots,
  \sigma(i+s+|p(\alpha_n)|, x_{\alpha_n}))$ that is
  $\sigma,i+s \models R(p(\alpha_1) ,\dots, p(\alpha_n))$ and $\sigma,i+s
  \models p(R(\alpha_1 ,\dots, \alpha_n)).$
In fact, if $\alpha = \aX^i x$ then $p(\alpha) = \aX^{i-s} x$ and
$|p(\alpha)| = |\alpha|-s$.
If $\alpha=  \aY^i x$ then $p(\alpha) = \aY^{i+s} x$ and
$|p(\alpha)| = -(i+s)=|\alpha|-s$, since $|\alpha| = -i$.

%\bigskip
\noindent {\bf Inductive step}.
% The {\bf inductive hypothesis} is $\sigma,i \models \psi \iFF \sigma,i+s \models p(\psi)$ for any subformula $\psi$ of $\phi$.
\begin{itemize}
\item If $\phi = \neg \psi$ then $\sigma, i \models \phi \iFF \sigma,i
  \not\models \psi$. By inductive hypothesis, this is equivalent to $\sigma,i+s \not\models p(\psi)$, i.e. $\sigma, i+s \models p(\phi)$, as $p(\phi) = \neg p(\psi)$.
\item If $\phi = \psi_1 \wedge \psi_2$ then $\sigma, i \models \phi
  \iFF \sigma,i \models \psi_1 \text{ and } \sigma,i \models
  \psi_2$. By inductive hypothesis, this is equivalent to $\sigma,i+s \models p(\psi_1) \text{ and } \sigma,i+s \models p(\psi_2)$, i.e. $\sigma, i+s \models p(\psi_1) \wedge p(\psi_2)$, and $\sigma, i+s \models p(\phi)$.
\item If $\phi = \X \psi$ then $\sigma, i \models \phi \iFF \sigma,i+1 \models \psi$. By inductive hypothesis, this is equivalent to  $\sigma,i+1+s \models p(\psi)$, i.e., $\sigma,i+s \models \X p(\psi)$, which corresponds to $\sigma, i+s \models p(\phi)$.
\item If $\phi = \Y \psi$ then $\sigma, i \models \phi \iFF \sigma,i-1 \models \psi$. By inductive hypothesis, this is the same as $\sigma,i-1+s \models p(\psi)$, i.e., $\sigma,i+s \models \Y p(\psi)$, and $\sigma, i+s \models p(\phi)$, as $p(\phi) = \Y p(\psi)$.
\item If $\phi = \psi_1 \U \psi_2$ then $\sigma, i \models \phi \text{ iff there exists } j\geq i \text{ s.t. } \sigma, j \models \psi_2 \text{ and }\sigma,n \models \psi_1  \text{ forall } i\leq n < j$, that is, by inductive hypothesis, $\sigma, j+s \models p(\psi_2) \text{ and } \sigma,n \models p(\psi_1) \text{ forall } i+s\leq n < j+s$, which in turn is equivalent to $\sigma, i+s \models p(\psi_1) \U p(\psi_2)$ and $\sigma, i+s \models p(\phi)$.
\item If $\phi = \psi_1 \Snc \psi_2$ then $\sigma, i \models \phi \text{ iff there exists } 0\leq j \leq i \text{ s.t. } \sigma, j \models \psi_2 \text{ and } \sigma,n \models \psi_1 \text{ forall } j < n \leq i$, that is, by inductive hypothesis $\sigma, j+s \models p(\psi_2) \text{ and } \sigma,n \models p(\psi_1) \text{ forall }\, j+s < n \leq i+s$, which is equivalent to $\sigma, i+s \models p(\psi_1) \Snc p(\psi_2)$ and $\sigma, i+s \models p(\phi)$.
\end{itemize}
%
Finally, $\sigma,0 \models \phi \siff \sigma, s \models p(\phi)$ by taking $i = 0$.
% Conversely, let $\sigma$ be a model for $\phi$ such that $\sigma,
% s \models p(\phi)$.
% First, consider the atomic
% formulae.
% Since $\sigma,i+s \models p(\alpha_1 \sim \alpha_2)$ then $\sigma,i+s
% \models p(\alpha_1) \sim p(\alpha_2)$ according to the rule given for $p$.
% This implies that $\sigma, i+s \models_\D \phi \iFF
% \sigma(i+s+|p(\alpha_1)|, x_{\alpha_1}) \sim
% \sigma(i+s+|p(\alpha_2)|, x_{\alpha_2})$.
% Equivalently, $\sigma, i+s \models_\D \phi \iFF
% \sigma(i+s+|\alpha_1|-s, x_{\alpha_1}) \sim \sigma(i+s+|\alpha_2|-s, x_{\alpha_2})$,
% that is $\sigma, i \models_\D \phi \iFF
% \sigma(i+|\alpha_1|, x_{\alpha_1}) \sim \sigma(i+|\alpha_2|, x_{\alpha_2})$.
% Formulae involving temporal operators and Boolean connective are
% treated similarly to the previous inductive step.
\qed
\end{proof} 

==> proof-proposition-LF.tex <==
\begin{proof}
Let us suppose that there exists an infinite (non strict) forward path $w$ in $\rho$, with $\alpha = \alpha' s$ and $\beta = \beta' s$.
Without loss of generality, we can consider $w$ to starts from $s$ ,
%because $w$ is infinite by iterating infinitely many times $\beta$
as $\alpha$ is a finite prefix.
%Let $n=|V|\cdot (-\lfloor\phi\rfloor+\lceil\phi\rceil+1)$ be the number of points within
%symbolic valuations.

%; then, it is possible to find a suitable
%position $j\leq t$ such that $p_{u+j|\beta|}\equiv p_u$.
Let us consider the word $s \beta^{t}$, where the suffix $\beta$ is repeated $t$
times, with $t$ large enough ($t$ is bounded by the number of all possible paths between two
points in $\beta$).
For all $i\ge 0$ and for all points $p$, let notation $p_i$ denote that $sv(p_i) = i$.
Let $u$ be the position of an occurrence of $s$ in $\rho$.
%and $\locfwdtc$ be the transitive closure of $\locfwd$.
We represent the sequence of points which are visited by $w$ at each occurrence of $s$ in $\rho$ as:
\[
p_u \fwd p_{u+|\beta|} \fwd \ldots \fwd p_{u+r|\beta|} \ldots
%p_u \locfwd^* p_{u+|\beta|} \locfwd^* \dots \locfwd p_{u+l|\beta|} 
\]
%where all points $p_{u+r|\beta|}$, with $r\in\interval{0}{t}$, are in $w$.
Since the number of points within symbolic valuations at each
position of $\rho$ is finite, then 
there exists a position $j \leq t$  such that $p_u\equiv
p_{u+j|\beta|}$; i.e., $w$, passing through $s \beta^{t}$, visits eventually point
$p_{u+j|\beta|}$ which is equivalent to $p_u$.
Hence, by transitivity $p_u\fwd p_{u+j|\beta|}$.
Moreover, let us consider all points $q_{u+l|\beta|}$, with
$l\in\interval{0}{t}$, such that $p_u \equiv q_{u+l|\beta|}$.
Then, because suffix $\beta$ is iterated and so are all the relations between
two points belonging to each $s \beta$ which occurs in $\rho$, and
because $p_u \fwd p_{u+j|\beta|}$ we have that $q_{u+l|\beta|} \fwd q_{u+(l+1)|\beta|}$ for
all $l\in\interval{0}{t-1}$ where each relation $\fwd$ between $q_{u+l|\beta|}, q_{u+(l+1)|\beta|}$ is witnessed by a path
within the corresponding occurrence of $s \beta$ which is recursively defined
as $q_{u+l|\beta|} \fwd \bar{p}_{u+l|\beta|} \fwd
q_{u+(l+1)|\beta|}$, for some $\bar{p}_{u+l|\beta|}$.
By definition of $\fwd$ over $\alpha' s \beta'
s$ we have $p\fwd p' = p\locfwd p'' \wedge p'' \fwd p'$ where points $p,p' \equiv p_u$ are
representative of all points $q_{u+l|\beta|}$, $sv(p)=loop-1$ and
$\rho'(loop-1)=s$, $sv(p')=k$ and $\rho'(k)=s$ and $p'' \equiv
\bar{p}_{u+l|\beta|}$.
% According to the definition of $F$, subpath $w'$ of $w$ starting
% from the symbolic valuation at position $k$ and obtained by $\beta^n$ is defined by:
% \[
% w' = (x,x')_{k}\cdot w_{x',y}\cdot
% (y,y')_{k+2|\beta|}\cdots (t,t')_{k+r|\beta|}\cdot w_{t',x} \dots %w_{x',z}\dots %(z,z')_{nk}
% \]
% where a pair $(v,v')_i$ represents the relation $p \locfwds p'$
% between two points (of the same symbolic valuation $i$) such that
% $var(p)=v$ and $var(p')=v'$ 
% and $w_{v',v''}$ is a forward
% path between two points $\triple{v'}{i}{h}$ and
% $\triple{v''}{j}{m}$ such that $i=loop-1$, $j=k$.
% Moreover, since there exists an infinite path induced by suffix
% $\beta$, there exists a pair $(u,u')_j$ of $w$ which is the same as
% $(z,z')_n$, with $1\leq j \leq nk$.
% For each pair $(x,x')_i$ we have
% $p \locfwds p'$, with $var(p)=x$, $var(p')=x'$; and for each path $w_{x, x'}$ we have
% $F(p,p')$, with $var(p)=x$, $var(p')=x'$ and $sv(p)=loop-1$, $sv(p')=k$, by definition of $F$ in (\ref{equation-definition-F}).
% Therefore, for each subpath $(x,x')_i\cdot
% w_{x',y}$ ($w_{x,y'}\cdot (y',y)_i$) we have $F(p,q)$, with $var(p)=x$, $var(q)=y$ and
% $sv(p)=loop-1$, $sv(q)=k$.
% Recursively, we obtain $F(p,p')$, with $var(p)=var(p')=x$ and
% $sv(p)=loop-1$, $sv(p)=k$, $shift(p)=shift(p')$.

Conversely, assume that $p\fwd p'$ holds (the case $p \fwds p'$ being analogous), with
$p=\triple{x}{loop-1}{h}$ and $p \equiv p'=\triple{x}{k}{h}$.
By
definition of $p\fwd p'$, there exists a finite number of points $p^1, p^2, \dots$ 
such that $p\locfwd p^1 \locfwd  p^2 \dots \locfwd p'$.
This forward path is 
visited infinitely many times, 
%F_{\alpha,\alpha}^{(\ell-1),k}(h,h) \iFF f_{\alpha,\gamma'}^{(\ell-1)}(h,m') \wedge F_{\gamma',\alpha}^{(\ell-1),k}(m',h).
% \]
% Hence, Recursively, each term $p'' \fwd p'$ entails
% a path from $p''$ to $p'$ such that $p'' \fwd p'$.
% %The infinite path visits infinitely often all points of the path $p\rightarrow p'' \rightarrow \dots \rightarrow p'$.
since $p\equiv p'$ and the suffix
$\beta$ is repeated infinitely often.
% sequence of points  $p\rightarrow
% p'' \rightarrow \dots \rightarrow p'$ 
Therefore, point $p$ and points equivalent to $p$ are visited infinitely many times in an infinite forward
path along $\rho=\alpha\beta^\omega$.
\end{proof}



==> proof-proposition-weak-symbolic.tex <==
\begin{proof}
First of all, it is straightforward to show that, if $v'$ is an assignment to terms (see Section \ref{section-symbolic}),
then, $v' \models_\D \fresh(sv)$ entails $v' \models_\D \fresh(\weak{sv})$.
Moreover,  if $v' \models_\D
f(\weak{sv})$ then there exists a symbolic valuation $sv'$, such that
$\weak{sv}'=\weak{sv}$ and $v' \models_\D f(sv')$.


Then, let $\set{V_1,\dots, V_h}$ be the partition of set $V$.

The first side is immediate, because all symbolic valuations in
$\rho$ contain relations between terms whose variables are not related
in $\phi$.
In particular, the symbolic valuations in $\rho$ involve $\D$-constraints
between variables belonging to different partitions of $V$.
Therefore, from $\sigma,0 \models \rho$ it descends $\sigma,0 \models \weak{\rho}$.
Moreover, $\weak{\rho},0\symodels\phi$ follows from the definition of
$\symodels$ with respect to atomic formulae
$R(\alpha_1,\dots,\alpha_n)$.
In fact, for all $i$ and $R(\alpha_1,\dots,\alpha_n)$ occurring in $\phi$, if $\rho,i\symodels R(\alpha_1,\dots,\alpha_n)$ then
$\weak{\rho},i\symodels R(\alpha_1,\dots,\alpha_n)$.

Conversely, suppose we have $\weak{\rho},0\symodels\phi \text{ and }
\sigma,0\models\weak{\rho}$.
Then, by Lemma \ref{lemma-A}, from $\sigma$ one can deduce a unique sequence of symbolic
valuations $\nu$ such that $\sigma,0\models \nu$.
%, by iterating the result for increasing values of $k$.
%Then, we immediately obtain that $\sigma,0\models \nu$.
As discussed in the first part of the proof, $\nu$ is a
symbolic model for formula $\phi$.
In fact, we observe that the weak version $\weak{\nu}$ of ${\nu}$ is exactly $\weak{\rho}$,
because both are such that $\sigma,0\models\weak{\rho}$ and
$\sigma,0\models\weak{\nu}$ (for each position they must exhibit the
same relation of $\phi$ between two -- or more -- terms).
Moreover, we have that $\nu,0\symodels\phi$ because $\weak{\nu},0\symodels\phi$ (recall $\weak{\nu} = \weak{\rho}$), and for all $i$ and $R(\alpha_1,\dots,\alpha_n)$ occurring in $\phi$, if
$\weak{\nu},i\symodels R(\alpha_1,\dots,\alpha_n)$, then 
$\nu,i\symodels R(\alpha_1,\dots,\alpha_n)$.
In other words, additional relations in symbolic valuations
occurring in $\nu$ (but not in $\phi$) do not affect the truth values of the relations occurring
in $\phi$.
\end{proof}

==> proof-theorem-removeAP.tex <==
\begin{proof}
We show that for all $i\geq 0$, $\pair{\pi}{\sigma},i \models \phi \iFF
r_{model}(\pi,\sigma),i \models (r(\phi) \wedge$ $
\G(\bigwedge_{i=1}^n (x_{p_i}=1)\vee (x_{p_i}=0)))$.
It follows immediately $\pair{\pi}{\sigma},i \models \phi \iFF
r_{model}(\pi,\sigma),i \models r(\phi) \text{ and }
r_{model}(\pi,\sigma),i \models \G(\bigwedge_{i=1}^n (x_{p_i}=1)\vee
(x_{p_i}=0))$.
Hereafter, we write $\theta$ instead of $r_{model}(\pi,\sigma)$.

First, we prove by induction the left subformula $\pair{\pi}{\sigma},i \models \phi \iFF
\theta,i \models r(\phi)$ for $i \geq 0$.
The {\bf base case} is given on propositional atoms.
Since $\pair{\pi}{\sigma},i \models p_j \iFF p_j \in \pi(i)$ and by
definition of $\theta=r_{model}(\pair{\pi}{\sigma})$, we can conclude
that $\theta(i,x_{p_j})=1$.
By definition $\theta,i\models (x_{p_j}=1) \iFF
\theta(i,x_{p_j})=1$; hence, $\theta,i \models r(p_j)$.
Moreover, because $\pair{\pi}{\sigma},i \models
R(\alpha_1,\dots,\alpha_n)$ depends only on $\sigma$ and
$\theta(j,x)=\sigma(j,x)$ for all $x \in V$ and $\lfloor\phi\rfloor \leq
j$, then $\theta,i \models R(\alpha_1,\dots,\alpha_n)$.

\noindent
{\bf Inductive step.}
\begin{itemize}
\item If $\phi = \neg \psi$ then $\pair{\pi}{\sigma}, i \models \phi
  \iFF \pair{\pi}{\sigma},i \not\models \psi$. By inductive
  hypothesis, this is equivalent to $\theta,i \not\models r(\psi)$,
  i.e. $\theta, i \models r(\phi)$, as $r(\phi) = \neg r(\psi)$. 
\item If $\phi = \psi_1 \wedge \psi_2$ then $\pair{\pi}{\sigma}, i \models \phi
  \iFF \pair{\pi}{\sigma},i \models \psi_1 \text{ and } \pair{\pi}{\sigma},i \models
  \psi_2$. By inductive hypothesis, this is equivalent to $\theta,i
  \models r(\psi_1) \text{ and } \theta,i \models r(\psi_2)$,
  i.e. $\theta, i \models r(\psi_1) \wedge r(\psi_2)$, and $\theta,
  i \models r(\phi)$.  
\item If $\phi = \X \psi$ then $\pair{\pi}{\sigma}, i \models \phi
  \iFF \pair{\pi}{\sigma},i+1 \models \psi$. By inductive hypothesis,
  this is equivalent to  $\theta,i+1 \models r(\psi)$, i.e.,
  $\theta,i \models \X r(\psi)$, which corresponds to $\theta, i
  \models r(\phi)$. 
\item If $\phi = \Y \psi$ then $\pair{\pi}{\sigma}, i \models \phi
  \iFF \pair{\pi}{\sigma},i-1 \models \psi \text{ and } i\geq 0$. By inductive
  hypothesis, this is the same as $\theta,i-1 \models r(\psi) \text{
    and }
  i\geq 0$, i.e., $\theta, i\models \Y r(\psi)$, and $\theta, i
  \models r(\phi)$, as $r(\phi) = \Y r(\psi)$. 
\item If $\phi = \psi_1 \U \psi_2$ then $\pair{\pi}{\sigma}, i \models
  \phi \iFF \text{there exists } j\geq i \text{ s.t. }
  \pair{\pi}{\sigma}, j \models \psi_2 \text{ and
  }\pair{\pi}{\sigma},n \models \psi_1  \text{ forall } i\leq n < j$,
  that is, by inductive hypothesis, $\text{there exists } j\geq i
  \text{ s.t. } \theta, j \models r(\psi_2)
  \text{ and } \theta,n \models r(\psi_1) \text{ forall } i\leq n <
  j$, which in turn is equivalent to $\theta, i \models r(\psi_1) \U
  r(\psi_2)$ and $\theta, i \models r(\phi)$. 
\item If $\phi = \psi_1 \Snc \psi_2$ then $\pair{\pi}{\sigma}, i \models \phi
  \iFF \text{there exists } 0\leq j \leq i \text{ s.t. } \pair{\pi}{\sigma}, j
  \models \psi_2 \text{ and } \pair{\pi}{\sigma},n \models \psi_1 \text{ forall }
  j < n \leq i$, that is, by inductive hypothesis $\text{there exists
  } 0\leq j \leq i \text{ s.t. } \theta, j \models
  r(\psi_2) \text{ and } \theta,n \models r(\psi_1) \text{ forall }\,
  j < n \leq i$, which is equivalent to $\theta, i \models
  r(\psi_1) \Snc r(\psi_2)$ and $\pair{\pi}{\sigma}, i \models r(\phi)$. 
\end{itemize}
Finally, we prove the first part $\pair{\pi}{\sigma},0 \models \phi \siff \theta,0
\models r(\phi)$, by taking $i = 0$.

Let us prove by induction the second part $\pair{\pi}{\sigma},i  \models
\phi \iFF \theta,i \models
\G(\bigwedge_{i=1}^n (x_{p_i}=1)\vee (x_{p_i}=0))$, for $i \geq 0$.
The {\bf base case} is $\theta,i \models \bigwedge_{i=1}^n (x_{p_i}=1)\vee
(x_{p_i}=0)$ which holds for all $i\geq 0$ by definition
of $r_{model}(\pi,\sigma)$.
The {\bf inductive hypothesis} applies on formula $\G(\bigwedge_{i=1}^n x_{p_i}=1)\vee
(x_{p_i}=0)$  at generic position $i$ for all $i\geq 0$.
$\theta,i \models \bigwedge_{i=1}^n (x_{p_i}=1)\vee
(x_{p_i}=0) \wedge \X\G(\bigwedge_{i=1}^n (x_{p_i}=1)\vee
(x_{p_i}=0))$
is equivalent to $\theta,i \models (\bigwedge_{i=1}^n (x_{p_i}=1)\vee
(x_{p_i}=0)) \text{ and } \theta,i \models \X\G(\bigwedge_{i=1}^n
(x_{p_i}=1)\vee (x_{p_i}=0))$.
The first conjunct follows from the base case.
The second formula $\theta,i \models \X\G(\bigwedge_{i=1}^n
(x_{p_i}=1)\vee (x_{p_i}=0))$ is equivalent to $\theta,i+1 \models \G(\bigwedge_{i=1}^n
(x_{p_i}=1)\vee (x_{p_i}=0))$ which holds by inductive hypothesis.
Therefore, by taking $i=0$ we conclude that $\theta,0 \models
\G(\bigwedge_{i=1}^n (x_{p_i}=1)\vee (x_{p_i}=0))$.
\end{proof}

==> section-related-tools.tex <==
\subsection{Tools for the time analysis of infinite state systems}
Recent results on infinite-state
verification are often associated with an intense activity of
tool development.

Decidability of Presburger arithmetic along with its relevance in
reducing problem like reachability and model-checking over counter
systems, has led to development of efficient tools for deciding satisfiability
of the full language $\PA$ or its fragments like quantifier-free $\PA$ or
$\DL$.
Omega library \cite{omega} is one of the best known candidate for
handling $\PA$ formulae.
% The Omega project has two major components. 
% One component is a system for manipulating sets of affine constraints over
% integer variables which
% was originally designed as a decision test for the
% existence of integer solutions to affine constraints. 
% Other than providing positive or negative answers to a satisfiability problem,
% the library constitutes of
% several routines for elimination of existentially quantified variables,
% elimination of redundant constraints, simplification of formulae
% involving negations and for verifying implications between formulae.
% The extended version of the Omega library
% is a complete system for simplifying and
% verifying Presburger formulas. 
The class of solvers for base theory include also Satisfiability
Modulo Theory solvers.
SMT-solvers implement different decision procedure for separated
theories and provide algorithms to solve satisfiability of
combination of them.
The Nelson-Oppen schema is one possible method for combining disjoint
theories.
However, many implemented algorithms exploit interaction with an
underlying SAT-solver: SMT instances are translated to
boolean SAT instances and first solved by a SAT
solver. 
This approach, which is referred to as the {\em eager} approach, has
the advantage of discovering immediately unsatisfiability derived from
boolean semantics of formulae.
On the other hand, the loss of the semantics of the underlying
theories may hinder the resolution of trivial facts.
This led to the development of a number
of SMT solvers which integrate Boolean reasoning of a
DPLL-style search with theory-specific solvers that handle
conjunctions of predicates from a given theory
({\em lazy} approach).
Not all SMT-solvers support quantifiers since they may lead to
undecidability.
We consider here the SMT features that sre most relevant in the context of our research.
The essential requirement that an SMT solver must satisfy to solve the $k$-bounded
satisfiability problem is the support for the theory of
uninterpreted functions and equality EUF combined with fragments of
arithmetic including $\triple{\Nat}{<}{=}$.
The following solvers provide the decision procedure for
quantifier-free EUF combined with Presburger arithmetic or Difference
Logic (thus, including $\triple{\Nat}{<}{=}$):
Microsoft Z3 (\url{http://research.microsoft.com/en-us/um/redmond/projects/z3/}), SRI
Yices (\url{http://yices.csl.sri.com/}), MathSat4
(\url{http://mathsat4.disi.unitn.it/}), Barcelogic
(\url{http://www.lsi.upc.edu/~oliveras/bclt-main.html}), CVC3
(\url{http://cs.nyu.edu/acsys/cvc3/}), OpenSMT (\url{http://verify.inf.usi.ch/opensmt}).
% \begin{description}
% \item[yices:] it is developed by SRI International. Yices decides the
%   satisfiability of propositional formulas that mix uninterpreted
%   function symbols and equality with interpreted symbols from the
%   following theories: linear real and integer arithmetic, arrays,
%   fixed-size bit-vectors, recursive datatypes, tuples, lambda
%   expressions and quantifiers. It also provides algorithm to produce
%   unsatisfiable core and maximal sat of formulae.
% \item[MathSat:] is a DPLL-based SMT-solver which supports theories of
%   equality and uninterpreted functions, linear real and integer
%   arithmetic and difference logic. It also supports unsatisfiable core algorithm.
% \item[z3:] equality over uninterpreted functions and
%   predicate symbols, real and integer arithmetic (with limited support
%   for non-linear arithmetic), bit-vectors, arrays,
%   tuple, records, enumeration types and algebraic (recursive)
%   data-types. It also supports partial decision procedure for
%   universal quantifier and non-linear arithmetic.
% \item[Barcelogic:] it is a DPLL-based SMT-solver which uses congruence
%   closure to solve EUF theory. It supports EUF and difference logic theories.
% \item[OpenSMT:] it is a DPLL-based SMT-solver which supports EUF,
%   difference logic and linear arithmetic over $\Zed$ and $\Q$ and
%   bit-vectors.
% \item[CVC3:] it works with several built-in theories: linear
%   arithmetic over $\Zed$ and $\Q$, arrays, tuples, records, inductive data types, bit
%   vectors, and equality over uninterpreted function symbols. It also supports quantifiers.
% \end{description}

Many solvers are integrated within high-level
verification tools which implement procedure for model-checking or
higher form of analysis like program analysis, secure programming development,
automatic systems synthesis, network protocols verification and
cryptography.
% \item[FAST:] \cite{BLP06} Fast is a tool for reachability/safety
%   verification of counter systems. It relies on symbolic
%   representation of both the systems and the specification which are
%   defined by Presburger formulae. The tool was first intended to handle flat
%   counter systems, for which symbolic representation of cycles
%   (acceleration) makes the procedure complete. Although many systems
%   do not have a flat representation, it is often possible to provide
%   an equivalent flat system with the same reachability set which can
%   be correctly verified. When flatness can not be exploited and
%   reachability set is not recursive, termination of the procedure can
%   be obtained by a user-guided interaction. Counter systems are
%   specified by means of a language defining control states and
%   transitions. Verification is done by computing backward and forward
%   analysis by means of functions $pre(t,S,k)$ and $post(t,S,k)$,
%   respectively, which computes the set of reachable configuration from
%   $S$ by using transitions defined in $t$ and by accelerating cycles
%   of length longer than $k$. For flat counter systems the two functions
%   compute the exact reachability set; when the system is not
%   flattable, both are semi-algorithms. Set theoretical functions
%   $\cup,\cap,\neg,\subseteq$ are used to 
%   manipulate set of configurations. For instance, reachability properties are
%   verified with $post(t,S,k)\subseteq GoodSet$ while safety is
%   verified by checking whether $pre(t,BadSet,k)\cap InitSet =
%   \emptyset$, where $GoodSet$ and $InitSet$ are two Presburger
%   definable sets of configurations.

As a first significant instance, we mention 
SAL (\url{http://sal.csl.sri.com/}) is a framework for specification and
  analysis of concurrent systems. It provides finite and infinite
  model-checker and other tools for checking deadlocks in finite
  concurrent systems and for generating random executions of
  finite and infinite state systems. The tool is aimed at verification
  of concurrent systems which are specified by a language allowing
  synchronous and asynchronous composition
  of interacting components. Finite model-checking is performed
  symbolically and also by explicit state algorithms, while infinite
  state verification is realized by $k$-inductive proof.
 Verification is tailored to
  clock-based automata, like Timed automata, endowed with infinite
  domain variables. In order to avoid the use
  of continuous clock, whose Zeno behavior (infinite occurrence of
  transitions without time progress) makes $k$-induction useless,
  timeout-based verification is realized by using time-progress
  transitions which update timeouts while discrete transitions are
  instantaneous since they leave time unchanged. Timeouts are temporal
  objects which store the time at which future discrete transitions
  will be taken. When an action occurs, since its timeout is elapsed,
  the action is realized and the timeout is updated to a new value,
  which is strictly larger than the current time. The benefit of
  timeouts is that they enforce a deterministic progress of
  time. There are no states in which both time-progress and discrete
  transitions are enabled. When a time-progress transition is enabled,
  time is advanced to the point where the next discrete transition is
  enabled. Therefore, all variables of the systems evolve in discrete steps.

Another high-level verification tool, Averest (\url{http://www.averest.org/}), 
is aimed to the 
  development of reactive systems. It
  consists of the various components: beside auxiliary modules, it
  provides a symbolic model checker and a tool for 
  hardware/software synthesis. The specification notation 
  includes a 
  synchronous languages (QUARTZ). Statements are ``executed'' as
  micro steps in zero time and time advancement is explicitly
  enforced by partitioning the micro steps of computation 
  into macro steps that take the same amount of logical
  time. Concurrent threads automatically
  synchronize at the end of a macro step. 
  Temporal specifications, given in
  linear temporal logic (LTL), are translated
  to $\omega$-automata and/or fixpoints in CTL and the
  $\mu$-calculus. Verification is provided by a symbolic
  model checker for finite and infinite state systems. Finite sets are
  encoded by their characteristic propositional functions which are
  represented by means of binary decision diagrams (BDDs)
  \cite{Bryant86} while infinite states are represented by Presburger
  arithmetic formulae. 

==> subsection-cltlb-cltl-equivalence.tex <==
\subsection{General equivalence result}
\label{subsection-cltlb-cltl-equivalence}


\input{indec}


Results proved in previous Sections help us to conclude the
equivalence between the language $\cltlb(L \cup \AP)$ and $\cltl{}{}(L)$
with only $\aX$.
\begin{theorem}\label{cltlb-cltl-equivalence}
Let $\phi$ be a $\cltlb(L \cup \AP)$ formula. Then, there exists an
initial equivalent $\cltl{}{}(L)$ formula $\phi'$ without $\aY$.
\end{theorem}
\begin{proof}
From Theorems \ref{theorem-removeY}, \ref{theorem-removeAP} we can
define $\phi'$ to be the composition 
of translation functions $r,p$, i.e., $\phi'= p(r(\phi))$.
Formula $\phi'$ belongs to $\cltlb(L)$ and its temporal modalities are
only $\X$, $\Y$, $\U$, $\Snc$ and $\aX$.
Then, from Theorem \ref{theorem-init-glob-equivalence}, formula
$\phi'$ is initially equivalent to a CLTL($L$) formula (with only $\aX$).
\end{proof}
